Score-Based Generative Modeling through Anisotropic Stochastic Partial Differential Equations

Score-based generative modeling (SBGM) has achieved state-of-the-art performance in image generation, with the quality of generated images being highly dependent on the design of the forward (diffusion) process. Among these, models based on stochastic differential equations (SDEs) have proven particularly effective. While traditional methods aim to progressively destroy all image information to enable reconstruction from pure noise, we propose a class of anisotropic stochastic partial differential equations (SPDEs) that preserve the geometric structure of the data over longer time scales throughout the transformation. These SPDEs consist of a drift term that enforces deterministic destruction via structured smoothing, and a diffusion coefficient that enables random destruction through noise injection. Both components are governed by anisotropy coefficients, enabling controlled, direction-dependent information degradation. This framework provides the theoretical foundation for a novel anisotropic score-based generative model. By retaining geometric structure for longer time scales, the backward generative process can exploit residual geometric cues, leading to improved reconstruction fidelity. We empirically validate this improvement in a proof-of-concept implementation on unconditional image generation, showing that anisotropic diffusion can achieve superior image quality metrics. We demonstrate consistent improvements in both pixel and latent space experiments over the SDE-driven baseline as well as over the state-of-the-art Flow Matching approach. Finally, we demonstrate the effectiveness of the introduced anisotropy in a conditional stroke-to-image generation task.

==> figures/alphas_comparison.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/alpha_comparison/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}

% \newcommand\scalevalue{0.645}    % 0.67, 0.82
\newcommand\scalevalue{0.9}    % 0.67, 0.82
\newcommand\scalevalueBigger{0.70}    % 0.67, 0.82


\small
\hspace*{-4mm}

% draw arrow
% \begin{tikzpicture}
% \begin{scope}
%     \draw [red,-{Stealth[width=2mm]}](1.27,0.37) -- (14.12,0.37) node[above]{\textcolor{black}{Forward process}};
%     % \fill [orange] (1.27,-0.37) rectangle (14.12,-1.37);
    
% \end{scope}
% \end{tikzpicture}

\begin{tabular}{c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;}}
%
~ &
$t=0$ &
$t=\frac{1}{8}T$ &
$t=\frac{2}{8}T$ &
$t=\frac{3}{8}T$ &
$t=\frac{4}{8}T$ &
$t=\frac{5}{8}T$ &
$t=\frac{6}{8}T$ &
$t=\frac{7}{8}T$ &
$t=T$ 
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Constant $\diffusivitytransition_1$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_1/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Increasing $\diffusivitytransition_1$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_1/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Constant $\diffusivitytransition_2$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_alpha_2/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Increasing $\diffusivitytransition_2$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_alpha_2/8.jpg}
\end{tikzpicture}
\\
%
% \\[-0.4mm]
% \rotatebox{90}{\hspace{0.1cm} \scriptsize Backward}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_6.jpg}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_5.jpg}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_4.jpg}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_3.jpg}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_2.jpg}
% \end{tikzpicture}
% &
% \begin{tikzpicture}[scale=\scalevalueBigger]
% \PlotSingleImage{backward/backward_1.jpg}
% \end{tikzpicture}
% \\[-0.4mm]
% \\


% \begin{tikzpicture}
% \begin{scope}
%     \draw [red,-{Stealth[width=2mm]}](1.27,0.37) -- (14.12,0.37) node[above]{\textcolor{black}{Forward process}};
%     % \fill [orange] (1.27,-0.37) rectangle (14.12,-1.37);
    
% \end{scope}
% \end{tikzpicture}

\end{tabular}



==> figures/bwd_process_vis.tex <==
\includegraphics[width=.5\textwidth]{example-image}

\includegraphics[width=.5\textwidth]{example-image-a}

\includegraphics[width=.5\textwidth]{example-image-b}

==> figures/diffusion/diffusion_coefficient_anisotropy_coefficient/diffusion_diffusion_coefficient_anisotropy_coefficient_small.tex <==
\begin{figure}[H]
    \vspace{-.6cm}
    \centering
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/intensity_coefficient/diffusion_intensity_coefficient_3.jpg}
        \caption*{$\anisotropytransition_2=\infty$}
    \end{minipage}
    \hfill
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusion_coefficient_anisotropy_coefficient/diffusion_diffusion_coefficient_anisotropy_coefficient_1.jpg}
        \caption*{$\anisotropytransition_2=1\mathrm{e-}2$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusion_coefficient_anisotropy_coefficient/diffusion_diffusion_coefficient_anisotropy_coefficient_2.jpg}
        \caption*{$\anisotropytransition_2=1\mathrm{e-}3$}
    \end{minipage}
    \caption{Comparison of different choices for the anisotropy coefficient $\diffusivitytransition_2$ of the diffusion coefficient $\diffusioncoefficient$. In all columns, we disabled the effect of the drift $\drift$ by setting $\diffusivitytransition_1=0$.}
    % \caption{Comparison of different choices for the anisotropy coefficients $\diffusivitytransition_2$ of the diffusion coefficient $\diffusioncoefficient$. The transformed image (originally depicted in \autoref{fig:diffusion-diffusivity-coefficient-comparison-small}) had a resolution of $128\times128$ pixels and the forward process was simulated up to time $\timepointmax=8$. In all columns, we disabled the effect of the drift $\drift$ by setting $\diffusivitytransition_1=0$. The image on the left is replicating the second column in \autoref{fig:diffusion-intensity-coefficient-comparison-small}, whereas the second image shows the effect of changing $\anisotropytransition_2$ from $\infty$ to $1\mathrm{e-}2$.}
    % \label{fig:diffusion-drift-anisotropy-coefficient-small}
    \vspace{-.3cm}
\end{figure}


==> figures/diffusion/diffusivity_coefficient/diffusion_diffusivity_coefficient_small.tex <==
\begin{figure}[H] % Force placement in one column
    \vspace{-8pt}
    \centering
    \begin{minipage}[t]{0.32\linewidth} % Adjust for 3 images
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusivity_coefficient/diffusion_diffusivity_coefficient_0.jpg}
        \par\vspace{\fill}
        \caption*{$\diffusivitytransition_1=0$}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusivity_coefficient/diffusion_diffusivity_coefficient_1.jpg}
        \par\vspace{\fill}
        \caption*{$\diffusivitytransition_1=1$}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusivity_coefficient/diffusion_diffusivity_coefficient_2.jpg}
        \par\vspace{\fill}
        \caption*{$\diffusivitytransition_1=.5\to8\cdot128$}
    \end{minipage}
    \caption{Comparison of different choices for the diffusivity coefficient $\diffusivitytransition_1$. The third column is using a \emph{geometric} transition of the form $\diffusivitytransition_1(\timepoint)=\diffusivitytransition_1^{\textnormal{min}}\left(\diffusivitytransition_1^{\textnormal{max}}/\diffusivitytransition_1^{\textnormal{min}}\right)^{\timepoint/\timepointmax}$ with $\diffusivitytransition_1^{\textnormal{min}}=1/2$ and $\diffusivitytransition_1^{\textnormal{max}}=8\cdot128$. In all columns, we disabled the effect of the diffusion coefficient $\diffusioncoefficient$ by setting $\diffusivitytransition_2=0$.}
    % \caption{Comparison of different choices for the diffusivity coefficient $\diffusivitytransition_1$. In all columns, we disabled the effect of the diffusion coefficient $\diffusioncoefficient$ by setting $\diffusivitytransition_2=0$. The third picture is using a \emph{geometric} transition of the form $\diffusivitytransition_1(\timepoint)=\diffusivitytransition_1^{\textnormal{min}}\left(\diffusivitytransition_1^{\textnormal{max}}/\diffusivitytransition_1^{\textnormal{min}}\right)^{\timepoint/\timepointmax}$.}
    \label{fig:diffusion-diffusivity-coefficient-comparison-small}
    \vspace{-6pt}
\end{figure}


==> figures/diffusion/drift_anisotropy_coefficient/diffusion_drift_anisotropy_coefficient_small.tex <==
\begin{figure}[H]
    \vspace{-.3cm}
    \centering
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/diffusivity_coefficient/diffusion_diffusivity_coefficient_2.jpg}
        \caption*{$\anisotropytransition_1=\infty$}
    \end{minipage}
    \hfill
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{figures/diffusion/drift_anisotropy_coefficient/diffusion_drift_anisotropy_coefficient.jpg}
        \includegraphics[width=\linewidth]{figures/diffusion/drift_anisotropy_coefficient/diffusion_drift_anisotropy_coefficient_1.jpg}
        \caption*{$\anisotropytransition_1=1\mathrm{e-}2$}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/drift_anisotropy_coefficient/diffusion_drift_anisotropy_coefficient_2.jpg}
        \caption*{$\anisotropytransition_1=1\mathrm{e-}3$}
    \end{minipage}
    \caption{Comparison of different choices for the anisotropy coefficient $\diffusivitytransition_1$ of the drift $\drift$. In all columns, we disabled the effect of the diffusion coefficient $\diffusioncoefficient$ by setting $\diffusivitytransition_2=0$.}
    % \caption{Comparison of different choices for the anisotropy coefficient $\diffusivitytransition_1$ of the drift $\drift$. The transformed image (originally depicted in \autoref{fig:diffusion-diffusivity-coefficient-comparison-small}) had a resolution of $128\times128$ pixels and the forward process was simulated up to time $\timepointmax=8$. In all figures, we disabled the effect of the diffusion coefficient $\diffusioncoefficient$ by setting $\diffusivitytransition_2=0$. The image on the left is replicating the third column in \autoref{fig:diffusion-diffusivity-coefficient-comparison-small}, whereas the second image shows the effect of changing $\anisotropytransition_1$ from $\infty$ to $1\mathrm{e-}2$.}
    \label{fig:diffusion-drift-anisotropy-coefficient-small}
    % \vspace{-20pt}
\end{figure}


==> figures/diffusion/intensity_coefficient/diffusion_intensity_coefficient_small.tex <==
\begin{figure}[H]
    \vspace{-.2cm}
    \centering
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/intensity_coefficient/diffusion_intensity_coefficient_1.jpg}
        \caption*{$\diffusivitytransition_2=1\mathrm{e-}2$}
    \end{minipage}
    \hfill
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/intensity_coefficient/diffusion_intensity_coefficient_2.jpg}
        \caption*{$\diffusivitytransition_2=1\mathrm{e-}1$}
    \end{minipage}
    \hfill
    %\begin{minipage}{0.48\linewidth}
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/diffusion/intensity_coefficient/diffusion_intensity_coefficient_3.jpg}
        \caption*{$\diffusivitytransition_2=1$}
    \end{minipage}
    \caption{Comparison of different choices for the intensity coefficient $\diffusivitytransition_2$. In all columns, we disabled the effect of the drift $\drift$ by setting $\diffusivitytransition_1=0$.}
    \label{fig:diffusion-intensity-coefficient-comparison-small}
    \vspace{-.3cm}
\end{figure}


==> figures/fid_error_plot.tex <==
\centering
\includegraphics[width=.40\textwidth]{figures/fid_error_plot/fid_convergence.jpg}

==> figures/lambdas_comparison.tex <==
%!TEX root = ../paper.tex

\newcommand{\PlotSingleImage}[1]{%
    % \begin{tikzpicture}[scale=1.165]
        \begin{scope}
            \clip (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
            \path[fill overzoom image=figures/lambda_comparison/#1] (0,0) rectangle (2.5cm,2.5cm);
        \end{scope}
        \draw (0,0) -- (2.5,0) -- (2.5,2.5) -- (0,2.5) -- cycle;
        
    % \end{tikzpicture}%
}

% \newcommand\scalevalue{0.645}    % 0.67, 0.82
\newcommand\scalevalue{0.9}    % 0.67, 0.82
\newcommand\scalevalueBigger{0.70}    % 0.67, 0.82


\small
\hspace*{-4mm}

% draw arrow
% \begin{tikzpicture}
% \begin{scope}
%     \draw [red,-{Stealth[width=2mm]}](1.27,0.37) -- (14.12,0.37) node[above]{\textcolor{black}{Forward process}};
%     % \fill [orange] (1.27,-0.37) rectangle (14.12,-1.37);
    
% \end{scope}
% \end{tikzpicture}

\begin{tabular}{c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;} c@{\;}}
%
~ &
$t=0$ &
$t=\frac{1}{8}T$ &
$t=\frac{2}{8}T$ &
$t=\frac{3}{8}T$ &
$t=\frac{4}{8}T$ &
$t=\frac{5}{8}T$ &
$t=\frac{6}{8}T$ &
$t=\frac{7}{8}T$ &
$t=T$ 
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Constant $\anisotropytransition_1$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_1/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Increasing $\anisotropytransition_1$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_1/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Constant $\anisotropytransition_2$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{cst_lambda_2/8.jpg}
\end{tikzpicture}
\\
\rotatebox{90}{\hspace{0.35cm} \scriptsize Increasing $\anisotropytransition_2$}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/0.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/1.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/2.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/3.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/4.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/5.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/6.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/7.jpg}
\end{tikzpicture}
&
\begin{tikzpicture}[scale=\scalevalueBigger]
\PlotSingleImage{inc_lambda_2/8.jpg}
\end{tikzpicture}
\\


\end{tabular}



==> figures/score_scaling_alpha.tex <==
% \includegraphics[width=.45\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}
% \includegraphics[width=.45\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}
% \includegraphics[width=.45\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}
% \includegraphics[width=.45\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}

\centering
\subfloat[$\weight(t)$ process 1]{\includegraphics[width=.40\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}}
\qquad
\subfloat[$\weight(t)$ process 2]{\includegraphics[width=.40\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}}
\qquad
\subfloat[$\weight(t)$ process 3]{\includegraphics[width=.40\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}}
\subfloat[$\weight(t)$ process 4]{\includegraphics[width=.40\textwidth]{figures/score_scaling_alpha/scaling_alpha_example.jpg}}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

